Constructing Set-Compositional and Negated Representations for First-Stage Ranking

Set compositional and negated queries are crucial for expressing complex information needs and enable the discovery of niche items like Books about non-European monarchs. Despite the recent advances in LLMs, first-stage ranking remains challenging due to the requirement of encoding documents and queries independently from each other. This limitation calls for constructing compositional query representations that encapsulate logical operations or negations, and can be used to match relevant documents effectively. In the first part of this work, we explore constructing such representations in a zero-shot setting using vector operations between lexically grounded Learned Sparse Retrieval (LSR) representations. Specifically, we introduce Disentangled Negation that penalizes only the negated parts of a query, and a Combined Pseudo-Term approach that enhances LSRs ability to handle intersections. We find that our zero-shot approach is competitive and often outperforms retrievers fine-tuned on compositional data, highlighting certain limitations of LSR and Dense Retrievers. Finally, we address some of these limitations and improve LSRs representation power for negation, by allowing them to attribute negative term scores and effectively penalize documents containing the negated terms.

==> method-rq2.tex <==
\subsection{Learning compositional representations from set compositional queries}\label{sec:method:rq2}
\added{\textbf{(TODO: remove entire subsection?)}}
In the previous section, we discussed how to derive compositional query representations for LSR based on atomic queries and their corresponding set-theoretic operations.
In this part, we probe the ability of different retriever families (LSR and DR) to learn effective set compositional representations for first stage ranking from training.

\subsubsection*{Ranking Loss}
Dense and Learned Sparse Retrievers are trained to map queries to relevant documents using a Ranking Loss. A very common option is Contrastive loss~\cite{}, that minimizes the distance between a query $q_i$ and a relevant document $d_i^+$, while maximizing the distance to irrelevant documents. Irrelevant documents contain negative documents for query $d_i^-$ and the positives of queries in the same batch $d_{i,j}^-$:
\[ \mathcal{L}_{Rank} = -log \frac{e^{s(q_i,d_i^+)}}{e^{s(q_i,d_i^+)} + e^{s(q_i,d_i^-)} + \sum{_j}e^{s(q_i,d_{i,j}^-)}} \]





